Noise suppression and long-range exchange coupling for gallium arsenide spin qubits

This thesis presents the results of the experimental study performed on spin qubits realized in gate-defined gallium arsenide quantum dots, with the focus on noise suppression and long-distance coupling.

==> CHAPTERS/Supplement_negative_J.tex <==
\chapterimage{Negative_J/fingerprint.png}
\chapter[Supplementary Information for ``Negative exchange interaction in a multielectron quantum dot'']{\protect\parbox{0.9\textwidth}{Supplementary Information for \\ ``Negative exchange interaction \\ in a multielectron quantum dot''}}
\label{ch:supp_negative-j}

\begin{center}
Frederico Martins$^{1,*}$, Filip K. Malinowski$^{1,*}$, Peter D. Nissen$^{1}$, \\
Saeed Fallahi$^{2}$, Geoffrey C. Gardner$^{3}$, Michael J. Manfra$^{2,3,4}$, \\
Charles M. Marcus$^{1}$, Ferdinand Kuemmeth$^{1}$
\end{center}

\begin{center}
	\scriptsize
	$^{1}$ Center for Quantum Devices, Niels Bohr Institute, University of Copenhagen, 2100 Copenhagen, Denmark\\
	$^{2}$ Department of Physics and Astronomy and Birck Nanotechnology Center, Purdue University, West Lafayette, Indiana 47907, USA\\
	$^{3}$ School of Materials Engineering and Birck Nanotechnology Center, Purdue University, West Lafayette, Indiana~47907, USA\\
	$^{4}$ School of Electrical and Computer Engineering, Purdue University, West Lafayette, Indiana 47907, USA\\
	$^{*}$ These authors contributed equally to this work
\end{center}

\begin{center}
\begin{minipage}{0.8\textwidth}
	\small
	...
\end{minipage}
\end{center}

